Flightmare: A Flexible Quadrotor Simulator

State-of-the-art quadrotor simulators have a rigid and highly-specialized structure: either are they really fast, physically accurate, or photo-realistic. In this work, we propose a novel quadrotor simulator: Flightmare. Flightmare is composed of two main components: a configurable rendering engine built on Unity and a flexible physics engine for dynamics simulation. Those two components are totally decoupled and can run independently of each other. This makes our simulator extremely fast: rendering achieves speeds of up to 230 Hz, while physics simulation of up to 200,000 Hz on a laptop. In addition, Flightmare comes with several desirable features: (i) a large multi-modal sensor suite, including an interface to extract the 3D point-cloud of the scene; (ii) an API for reinforcement learning which can simulate hundreds of quadrotors in parallel; and (iii) integration with a virtual-reality headset for interaction with the simulated environment. We demonstrate the flexibility of Flightmare by using it for two different robotic tasks: quadrotor control using deep reinforcement learning and collision-free path planning in a complex 3D environment.

==> tables/rl_tasks.tex <==
\begin{table}[!htp]
    \centering
    \begin{tabular}{l|c|r} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
      \textbf{Value 1} & \textbf{Value 2} & \textbf{Value 3}\\
      $\alpha$ & $\beta$ & $\gamma$ \\
      \hline
      1 & 1110.1 & a\\
      2 & 10.1 & b\\
      3 & 23.113231 & c\\
    \end{tabular}
    \caption{Your first table.}
    \label{tab:table1}
\end{table}

==> tables/sim_comparison.tex <==
\begin{table}[!htp]
	\centering
	\resizebox{\columnwidth}{!}{%
        \begin{tabular}{|p{2cm}||p{1.5cm}|p{1.5cm}|p{0.6cm}|p{0.6cm}|p{0.6cm}|p{0.75cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|}
        	\hline
        	Simulator & Rendering Engine & Physics Engine & IMU & RGB & Depth & OF & OS & CS & L & PC & VR \\
        	\hline
        	RotorS & Gazebo &  & x & x & x & (x) & (x) & (x) & (x) & x & -\\
        	Hector & Gazebo &  & x & x & x & (x) & (x) & (x) & x & x & -\\
        	AirSim & Unreal &  & x & x & x & x & x & - & x & - & -\\
        	FlightGoggles & Unity &  & x & x & x & - & - & - & x & - & x \\
        	\hline
        	\textbf{Flightmare} & \textbf{Unity} &  & \textbf{x} & \textbf{x} & \textbf{x} & \textbf{x} & \textbf{x} & \textbf{x} & \textbf{x} & \textbf{x} & \textbf{x}\\
        	\hline
        \end{tabular}
        }
	\caption{A comparison of Flightmare and other open source quadrotor simulator. }
\label{tab:simulators}
\end{table}
